Towards Feasible Counterfactual Explanations: A Taxonomy Guided Template-based NLG Method

Counterfactual Explanations (cf-XAI) describe the smallest changes in feature values necessary to change an outcome from one class to another. However, many cf-XAI methods neglect the feasibility of those changes. In this paper, we introduce a novel approach for presenting cf-XAI in natural language (Natural-XAI), giving careful consideration to actionable and comprehensible aspects while remaining cognizant of immutability and ethical concerns. We present three contributions to this endeavor. Firstly, through a user study, we identify two types of themes present in cf-XAI composed by humans: content-related, focusing on how features and their values are included from both the counterfactual and the query perspectives; and structure-related, focusing on the structure and terminology used for describing necessary value changes. Secondly, we introduce a feature actionability taxonomy with four clearly defined categories, to streamline the explanation presentation process. Using insights from the user study and our taxonomy, we created a generalisable template-based natural language generation (NLG) method compatible with existing explainers like DICE, NICE, and DisCERN, to produce counterfactuals that address the aforementioned limitations of existing approaches. Finally, we conducted a second user study to assess the performance of our taxonomy-guided NLG templates on three domains. Our findings show that the taxonomy-guided Natural-XAI approach (n-XAI^T) received higher user ratings across all dimensions, with significantly improved results in the majority of the domains assessed for articulation, acceptability, feasibility, and sensitivity dimensions.

==> ap-additional-content.tex <==
\section*{Supplementary Material}

Sample responses from participants of user study 2 who viewed explanations generated with (\nxai) and without (\basexai) feature actionability knowledge. Also, All the code for the proposed method, along with the necessary documentation, is available in our online code repository\footnote{https://anonymous.4open.science/r/NLGXAI-0BC6/src/inference.py}.


\begin{table}
\centering
\scalebox{0.78}{
\begin{tabular}{lll}
\hline
Dataset & Explanation with \nxai & Explanation with \basexai \\ \hline
Heart Disease & \begin{tabular}[c]{@{}l@{}}In order to prevent heart problems you would need to change 5 attributes.\\ You would not have heart disease if you,\\ 1), take steps to reduce resting blood pressure to 94.0 and,\\ 2), decrease serum cholesterol from 471.0 to 248.0.\\ 3), raise thalach from 122 to 132.0.\\ 4), increase old peak from 1.0 to 2.0.\\ 5), raise ca from 0 to 1.0.\\ Furthermore, Your age has contributed to having a heart problem.\\ Moreover, sex Male has a higher chance to have a healthy heart compared to\\ sex Female and, stay safe!\end{tabular} & \begin{tabular}[c]{@{}l@{}}In order to prevent heart problems you would need to change 7 attributes.\\ You would not get heart problems if you,\\
1), decrease age to 33.0 and,\\ 2), change sex to Male and,\\3), raise resting blood pressure to 108.0 and,\\ 4), increase chol to 525.0 and, \\ 5), lower thalach to 75.0 and,\\ 6), reduce old peak to 0.0 and, \\7), reduce thal to 0.0. Take care!\end{tabular} \\ \hline
Credit Risk & \begin{tabular}[c]{@{}l@{}}To reduce your credit risk, you would need to change the following 4 attributes.\\ 1), take steps to raise Annual Income to 12000.0 and, \\ 2), take steps to modify Home ownership to RENT and, \\ 3), raise Loan amount to 1600.0. \\ 4), decrease Interest rate to 10.59. \\ In addition, individuals with Employment length 3.0 has a higher chance to have\\ a risk free credit compared to individuals with Employment length 5.0. \\ Wishing you a successful financial journey where your credit remains protected!\end{tabular} & \begin{tabular}[c]{@{}l@{}}To reduce your credit risk, you would need to change the following 5 attributes.\\ 1), raise Annual Income to 12000.0 and,\\ 2), modify Home ownership to RENT and, \\ 3), raise Loan amount to 1600.0 and, \\4), decrease Interest rate to 10.59 and, \\5), decrease Employment length to 3.0.\\ Wishing you a successful financial journey where your credit remains protected!\end{tabular} \\ \hline
Student Performance & \begin{tabular}[c]{@{}l@{}}In order to get a total score that is above the average, you would need to \\ change the following 3 attributes.\\ 1), increase math score to 68.0. \\ 2), raise reading score to 72.0. \\ 3), increase writing score to 64.0. \\ Furthermore,  parental level of education is a contributing factor to the risk\\  of obtaining an overall score of below the average. Good luck with your results!\end{tabular} & \begin{tabular}[c]{@{}l@{}}In order to get a total score that is above the average, you would need to change\\ the following 4 attributes.\\1), increase math score to 68.0 and, \\2), raise reading score to 72.0 and, \\3), increase writing score to 64.0 and,\\ 4), change your parental level of education to bachelor's degree. Good luck with your results!\end{tabular} \\ \hline
\end{tabular}
}
%
\caption{A sample of responses for \nxai and \basexai.}
\label{tab:userstudy2}
\end{table}

In our second user study, we asked participants a series of questions addressing four criteria: articulation, acceptability, feasibility, and sensitivity. These questions appear in Table \ref{tab:us2Qs}. Additionally, we also asked them to explain their reasons for their choices in an open-ended question.
\begin{table}
\centering
\begin{tabular}{ll}
\hline
\textit{Criteria} & \textit{Questions} \\ \hline
Articulation & \begin{tabular}[c]{@{}l@{}}On a scale of 1 to 5, with 1 being "strongly disagree" and 5 being "strongly agree", \\ how would you rate the statement: "Regardless of accuracy, this explanation is well articulated"?\end{tabular} \\ \hline
Acceptability & \begin{tabular}[c]{@{}l@{}}On a scale of 1 to 5, with 1 being "not at all acceptable" and 5 being "completely acceptable", \\ how would you rate the acceptability of the counterfactual explanation provided to the user?\end{tabular} \\ \hline
Feasiblity & \begin{tabular}[c]{@{}l@{}}On a scale of 1 to 5, with 1 being "not at all feasible" and 5 being "completely feasible", \\ how would you rate the feasibility of the counterfactual explanation provided to the user?\end{tabular} \\ \hline
Sensitivity & \begin{tabular}[c]{@{}l@{}}On a scale of 1 to 5, with 1 being "strongly disagree" and 5 being "strongly agree", \\ to what extent do you believe that sensitive personal characteristics and ethical considerations\\  are appropriately addressed in the counterfactual explanation provided?\end{tabular} \\ \hline
\end{tabular}
\caption{Questions related to 4 criteria of evaluating \nxai}
\label{tab:us2Qs}
\end{table}

==> ap-user-study-1.tex <==
\section{User study 1}
\label{ap:user-study-1}

% \subsection{Textual representation generation}

% points to cover:

% 1. what are the templates

% 2. some examples

% 3. table 1 column Cohort 2(provided) and analysis 

% 4. table 2 column cohort 2 (provided) and analysis
% \subsubsection{Templates used in first user study}
% we utilized two initial templates for converting counterfactual explanations into natural language. The first template employed feature grouping based on their action type, while the second template ordered features according to their importance using SHAP values. Table \ref{tab:initialTpls} show an example of an explanation using both templates.

% \subsection{Storyboard}
% Figure \ref{fig:screenshot} illustrates the storyboard comprising pages incorporated into the first user study website. Google Sites was utilized for the creation of this initial study.

% \subsection{User Study 1: Cohort Response Examples}
% Table \ref{tab:us1cohortsResponses} presents examples of responses from the cohorts in User Study 1, highlighting the variety of explanations provided by participants.


==> introduction.tex <==
\section{Introduction}
\label{introduction}
% Talk about CF requirements then aspects lit didn't cover (feasibility and its branches) - checked

%As artificial intelligence (AI) systems become increasingly integrated into our daily lives, the need for transparency and interpretability of these systems grows. 
Counterfactual explanations have emerged as a promising solution for providing users with a better understanding of the underlying reasoning behind the output of black-box AI models ~\cite{wachter2017counterfactual,keane}. In a counterfactual explanation, the user is shown how the output of the model would have changed if one or more input features had been different.
% Counterfactual Explanations Goals
In this context, \cite{wachter2017counterfactual} propose three goals for explanations: (1) inform and clarify the reasoning behind decisions, (2) give the explainee sufficient information to question or object to decisions that negatively impact them, and (3) enable understanding of required changes for desired future results, given the current decision-making model.

%Generally, in order to provide effective and meaningful counterfactual explanations, it is crucial that specific requirements be met. 
A good counterfactual is both proximal and sparse, allowing explainers to pinpoint the closest favorable outcomes while necessitating value changes to a minimal set of features ~\cite{keane2020good}. 
While state-of-the-art explainers~\cite{discern, nice, dice} emphasise these requirements, it is important to extend the focus of counterfactual explanations 
to carefully consider the feasibility of proposed feature changes, particularly accounting for properties like immutability (e.g., suggesting a change to one's age).
Additionally, adhering to distributional faithfulness is essential for upholding the plausibility of counterfactuals, warranting that the produced explanations remain within the bounds of realistic and credible possibilities (e.g., expected age range). 
To meet these requirements for good counterfactuals, it is essential to carefully assess the feasibility of proposed feature changes within the user's context and also to consider their appropriateness in adhering to ethical considerations (e.g., suggesting changes to race).
%However, creating effective counterfactual explanations requires careful consideration of the relevant features, their feasibility, and the user's goals and personalisation, as well as ethical implications.

In this paper, we present a novel approach for generating feasible counterfactual explanations in natural language. 
Our work builds upon a user study conducted to identify key factors considered by humans when crafting counterfactual explanations. 
Our analysis of user feedback identified seven key themes, which we broadly categorised according to their relation to content or structure. Using these themes, we developed an extendable taxonomy of feature feasibility with four categories: directly mutable, indirectly mutable, regular immutable, and sensitive immutable. 
Additionally, we created a generalisable, template-based text generation pipeline that employs the feasibility taxonomy to handle features appropriately. 
This NLG pipeline is compatible with existing counterfactual explainers such as DICE, NICE, and DISCERN.
%This taxonomy allows for the careful consideration of ethical implications and biases across different domains, such as health, education, and finance.
%These methods generate counterfactual explanations in natural language that are not only plausible but also ethically sound and feasible.
%Recognising the need for a more systematic approach to addressing feasibility, ethics, and biases, 

This paper addresses the following research questions related to counterfactual explanations in natural language:
\begin{itemize}
    \item RQ1: What are the key factors and common constructs that contribute to plausible and understandable counterfactual explanations in natural language?
    \item RQ2: How can the identified factors be used to create a generalisable, ethical, and human-centric approach for counterfactual explanation generation across different domains?
\end{itemize}

Our contributions include:

\begin{itemize}
    \item Findings from a user study aimed at identifying requirements for generating natural language explanations for counterfactual scenarios;
    \item Introduction of a taxonomy for classifying feasibility on the basis of immutable and mutable categories for counterfactual XAI, taking into account ethics and biases;
    \item Development of a template-based language generation approach for counterfactual explanations that incorporate the taxonomy and insights from our user study;
    \item Demonstration of the effectiveness of the template-based Natural Language Generation (NLG) approach by conducting a second user study to assess its performance in terms of biases, ethics, acceptability, feasibility, and articulation.
\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=0.38\textwidth]{diagram.png}
    \caption{Counterfactual explanation pipeline in natural language}
    \label{fig:pipeline}
\end{figure}

%Overall, our work contributes to the ongoing effort to improve the transparency and interpretability of AI systems and to build AI systems that are trustworthy and aligned with human values and goals.
In the rest of the paper, we discuss related work in Section~\ref{relatedworks}, with details of the first user study appearing in~\ref{userstudy}. 
Findings and insights from the user study shape how actionable instructions from counterfactual XAI must be presented and these are formalized in the taxonomy in Section~\ref{taxonomy}. The templates derived for each of the leaf nodes and the manner of combining template constructs are presented in Section~\ref{Templates} followed by an evaluation by conducting the second user study in Section~\ref{userstudy2} and finally our conclusion and future works. Figure \ref{fig:pipeline} illustrates the pipeline of generating counterfactual explanations employing feasibility taxonomy in natural language.

==> old_us1.tex <==
\section{User Study 1: Understanding how people write counterfactuals}
\label{userstudy}

% RQ1: What are the language constructs commonly used when expressing counterfactual explanations?

We conducted a user study with the aim of collecting natural language descriptions of counterfactual explanations written by humans. 
The purpose of this study was to analyze these descriptions and identify language constructs commonly used when expressing counterfactual explanations. To achieve this goal, we used the loans dataset, which is a commonly used dataset for exploring counterfactuals.

The survey was administered through web pages, with participants first presented with information about the dataset's features. They were then presented with five examples of rejected loan applicants, each with a corresponding counterfactual generated by the DiCERN algorithm \cite{discern}. To provide participants with a manageable task within a short timeframe, the counterfactuals presented had four or five changes. We chose these numbers based on an analysis of the distribution of feature changes in 3000 different samples, where four and five changes were the most common. Figure \ref{fig:featchanges} illustrates the distribution of feature changes across 3000 samples.

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{changed_feature_hist.png}
    \caption{Distribution of Changed Features across 3000 Samples}
    \label{fig:featchanges}
\end{figure}
Participants were asked to write an English description that they would provide to the loan applicant based on the provided counterfactual. To explore the impact of different counterfactual presentation modes, participants were split into two cohorts: cohort one participants were presented with tables and graphs, while cohort two participants were presented with two textual descriptions generated by two simple templates.

After writing each counterfactual description, participants were asked to rank the type of explanations provided to them in terms of usefulness and provide reasons for their selection and ordering. This allowed us to gain insights into the factors that participants considered important when evaluating counterfactual explanations.

The user study provided us with a dataset of natural language descriptions of counterfactual explanations, which we plan to analyze to identify common patterns that can be used to create counterfactual explanation templates. Additionally, our study explored the impact of different counterfactual presentation modes on user comprehension and perception of usefulness.
\subsection{Participants}
Participants(N=33) for this user study were students in the school of computing. Different websites of each cohort were distributed randomly among them.
\subsection{Quantitative Evaluation}
We begin our first phase of analysis by filtering out responses that were deemed not useful due to factors such as the descriptions being too short or the participants not following the instructions and responding out of context. After this filtering process, we were left with a total of 109 samples that we used in our analysis. This step was necessary to ensure that we only analyzed responses that provided meaningful insights into our research question. Out of a total of 109 samples, 55 were from the first cohort and the rest were from the second cohort. The shortest generated text by users was two words long, while the longest was 209 words long, and the average generated explanation was 33 words long. The above information for each cohort is depicted in table \ref{table:1}.
\begin{table}
\centering
\begin{tabular}{|l|l|l|l|l}
\hline
                  & Cohort 1 & Cohort 2 & Cohort 2 (provided) \\ \hline
Number of samples & 55       & 53       & 14       \\ \hline
Minimum Length    & 2        & 4        & 241       \\ \hline
Maximum Length    & 209      & 75       & 303      \\ \hline
Average Length    & 35       & 30       & 278.71       \\ \hline

\end{tabular}
\caption{Distributional information about each cohort}
\label{table:1}
\end{table}

We analyzed and compared generated texts of each cohort in four different criteria as follows:
\begin{enumerate}
    \item Ease of Readability employing Flesch Score
    \item Grammatical Error Analysis
    \item Token-wise similarity of each text with our ground truth textual explanations provided in cohort
    \item Semantic similarity of texts with their corresponding ground truths

\end{enumerate}

\subsubsection{Readability}
We use the Flesch score \cite{flesch1948new} to assess readability, which measures the ease of readability as well as text level. According to our observations, explanations from cohort 1 were fairly difficult, particularly at level 10, where cohort 2 explanations were difficult, and at the college level, where they generated more advanced explanations than cohort 1 users. Readability results are shown in table \ref{table:2}.

\begin{table}
\centering
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{}             & \textbf{Cohort 1} & \textbf{Cohort 2} & \textbf{Cohort 2 (Provided)} \\ \hline
\textbf{Flesch Score} & 52.79             & 41.93            & 19.89 \\ \hline
\textbf{Ease Score}   & Fairly Difficult  & Difficult       & very confusing         \\ \hline
\textbf{Level}        & 10                & College        & college-graduate   \\ \hline
\end{tabular}
\caption{Average readability scores of each cohort}
\label{table:2}
\end{table}

\subsubsection{Grammatical Error Analysis}
In addition to our analysis of the natural language descriptions, we also conducted a grammatical error analysis using the python language tool library \footnote{https://pypi.org/project/language-tool-python/}. The aim of this analysis was to investigate whether participants were bothered by grammatical errors in their descriptions and whether there were any differences in the number of grammatical errors between the two cohorts.

It is worth noting that participants were entering text into a web form without any automated support, which could have led to more grammatical errors. Therefore, we were interested in exploring whether this lack of support had an impact on the quality of the participants' descriptions.

By conducting this analysis, we gained insights into the extent to which participants were able to produce grammatically correct descriptions and whether there were any differences in this regard between the two cohorts.

Analysis of grammatical errors has been the subject of several studies \cite{grammaticalErr}. We thus made the decision to apply this analysis to the data we had gathered to see if the users' grammatical performance would be affected by just seeing graphs and tables rather than text summaries.
Grammatical error analysis in both cohorts reveals that in cohort 2, there were 18 mistake-free explanations compared to 16 in cohort 1. Furthermore, the highest number of mistakes in cohort 1 was 8, compared to 7 in cohort 2. Firstly, it suggests that the format of the counterfactual explanation can have an impact on the quality of the natural language descriptions that users produce. In this case, textual explanations seem to have led to better-quality descriptions, which can be an important consideration when designing future user studies or counterfactual explanation systems.

Secondly, it indicates that providing clear and concise textual templates can be an effective way to guide users in producing high-quality natural language descriptions. This can help to ensure that the descriptions provided are meaningful and useful for the purpose of analyzing common patterns and extracting templates.

Lastly, it highlights the importance of considering user experience and usability when designing counterfactual explanation systems. By presenting information in a way that is easy to understand and process, users are more likely to engage with the system and produce high-quality outputs, which can ultimately improve the effectiveness and impact of the system.
\subsubsection{Token-wise Similarity}
To validate the aforementioned analysis, we performed a token-wise similarity check between explanations written in both cohorts and ground-truth explanations provided in cohort 2 for each customer. The results demonstrate that the total similarity between cohort 1 explanations and ground-truth explanations was only 7 percent, which is understandable given that they did not witness such explanations, but the similarity between ground-truth explanations and cohort 2 is only 23 percent, indicating that small copying footsteps occurred.

\subsubsection{Semantic Similarity}
In order to broaden the prior analysis, we do a semantic similarity check using the all-MiniLM-L6-v2 model from the sentence-transformers framework \cite{reimers-2019-sentence-bert}. The results for semantic similarity demonstrate that cohort 1 has a semantic resemblance with ground-truth explanations which was on average 55.4 percent, whereas cohort 2 has a semantic similarity of 70.28 percent. 
According to the results, there are a number of explanations that were replicated from the offered explanations, but the extraction of a decent template requires more qualitative examination.

\subsection{Qualitative Evaluation}
%
%
\begin{table*}[!htb]
\centering
\footnotesize
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{p{3.5cm}p{7cm}cp{2cm}}
\hline
Themes & Example & Frequency & Corresponding cluster(s) \\
\hline
1. Vague explanation & The customer should lower their collection fee and their recoveries as well as increase their total payment and their principal & 23 & 1, 4, 5, 3 \\
2. Only considering counter-factual values & For your application to be improved, you would need to increase total\_pymnt to 12268.08 and total\_rec\_prncp to 10925.You would need to decrease recoveries and collection\_recovery\_fee to 0. & 39 & 0, 2 \\
3. Considering both counter-factual and query values & For your application to be successful you should increase you total payment to 12268.08 from 5040.00 while also increasing your principal to 10925.00 from 1492.93 and decrease recoveries and recovery collection fee to 0. & 5 & 0, 2 \\
4. Mixture of using counter-factual and query values & They need to pay more in, reduce the recoveries to 0 \& principal needs to be bigger & 3 & 0, 2 \\
5. Using ordinal adverbs / Bullet-pointing & For your application to be accepted, you will need to prioritize the following in the order given: 1) increase the total principal received (total\_rec\_prncp) to 14,999 2) decrease the recoveries (recoveries) to 0.00 3) decrease the collection recovery fee (collection\_recovery\_fee) to 0.00  4) increase the last payment amount (last\_pymnt\_amnt) to 11,448.66 & 12 & 2 \\
6. Simplified explanation & Increase your last payment amount and recoveries to 0 & 20 & 0, 5 \\
7. Using a wide range of terms (e.g. changing words) & Customer 1 should pay off their recoveries and negotiate to have their charge off removed & 4 & 2 \\
\hline
\end{tabular}
\caption{Comparison of manual data analysis and Agglomerative Clustering.}
\label{tab:user-study-discussion}
\end{table*}


%
%it is a user study of which results were analysed using a thematic analysis. 
Quantitative results so far have shown that individuals who only saw textual explanations constructed better explanations compared to those who saw both graphical and tabular explanations. This suggests that textual explanations may be more effective at conveying information and facilitating understanding compared to other forms of presentation. It is worth noting that these findings may be specific to the particular task and dataset used in the study, and further research is needed to determine the generalizability of these results. Nonetheless, these findings highlight the potential value of focusing on the development of text-based explanation methods in certain contexts.
More qualitative studies are required to obtain a good template.
Our qualitative evaluation consists of two steps. In the first step, we analyzed all explanations manually and classified them into seven different themes then we conduct a clustering to compare automatically created clusters with our themes.
\subsubsection{Manual Analysis}
These explanations were manually analyzed and divided into different themes as follows:
1. Some users used vague language in their counterfactual explanations, meaning that they did not mention any numerical values to indicate how much a certain feature value should be changed.
2. Other users only mentioned the counterfactual values and not the query values, meaning that they provided the desired values for the features but did not specify the current values.
3. Some users mentioned both the query and counterfactual values, providing both the current and desired values for the features.
4. Some users used a mixed approach, including both query and counterfactual values for some features and only counterfactual values for others.
5. Some users employed ordinal adverbs or bullet pointing in their explanations, using words like "first" or "second" to indicate the order of the changes or using bullet points to list the changes.
6. Other users wrote simplified explanations, using simpler language and fewer details.
7. Finally, some users used a wide range of terms and words to describe the changes, including synonyms like "increase" and "raise" to describe the same concept.
 
 Upon closer examination of the natural language explanations provided by the participants in our user study, we found evidence that suggests that users attempted to interpret the rejected loan applicant's situation and understand the underlying reasons for their rejection. Specifically, our analysis revealed that participants in categories 1, 5, 6, and 7 often included some level of interpretation of the query or counterfactual values, such as explaining the need for changing a particular feature as well as considering the actionability of particular features in their interpretation in order to improve the applicant's chances of being approved. In contrast, participants in categories 2, 3, and 4 tended to focus solely on the values that needed to be directly changed without providing any additional interpretation or context. These findings highlight the importance of understanding how users interpret counterfactual explanations and suggest that improving the design and effectiveness of the templates can help users make better decisions in complex decision-making scenarios.
\subsubsection{Cluster Analysis}
Next, agglomerative clustering was used to cluster the explanations to check if it validates our manually extracted themes. The average linkage method is used to merge the clusters based on their similarity. The explanations were encoded using the  pre-trained all-MiniLM-L6-v2 model from the sentence transformers library to create embeddings, which were used as input to the clustering algorithm. The resulting clusters were then compared to the themes identified through manual analysis in order to assess the similarity between the two. The results of the analysis are shown in table \ref{tab:user-study-discussion}.

Our analysis using agglomerative clustering revealed interesting patterns among the themes identified in our user study. Specifically, we found that themes 2, 3, 4, 5, and 7 were highly similar and mostly clustered together in cluster 0 and 2. On the other hand, theme 1 and a portion of theme 6 were grouped together in clusters 1, 4, 5, and 3. Notably, these clusters contained explanations that were simplified and vague, without explicitly mentioning any values, revealing that Our agglomerative clustering results were consistent with our manually extracted themes. 

\subsection{Addressing RQ1: What are the key factors and common constructs that contribute to effective and understandable counterfactual explanations in natural language?}

In our study, we analyzed the generated explanations and classified them into 7 distinct themes based on their specific style of explanations. We then conducted agglomerative clustering to compare these selected themes with themes generated by the clustering algorithm to validate our manually extracted themes.

To further elaborate on how the user study has influenced the creation of new templates, we took a more holistic approach to design the templates by considering the best aspects of each theme and cluster. This included using a wide range of terms to increase the diversity of explanations, incorporating some level of interpretation to provide a better understanding of the reasoning behind the recommendations, considering feature actionability using ordinal adverbs to make the explanations clear, and also including numerical values to improve understandability. While the inclusion of numerical values was influenced by the observation that most users tended to include them in their explanations, we also recognized that vague language could be useful for certain features, particularly when discussing their actionability. By taking into account the advantages of each theme and cluster, we believe that our new templates are better suited to meet the needs of a wide range of users in complex decision-making scenarios.

In the next section, we will employ the insights extracted from our user study to address RQ2 by designing a taxonomy for feature actionability and consequently, we are going to construct appropriate templates to develop a solution for generating counterfactual explanations. This template-based approach represents a promising direction for generating natural language explanations that are both accurate and understandable to end users. By leveraging the insights gained from our user study, we aim to create a method that is effective at generating counterfactual explanations in a way that is both clear and understandable to the user.

==> reusable.tex <==
\begin{table*}[]
\tiny
\centering
\begin{tabular}{llll}
\hline
Dataset & Metric & Explanation with actionability taxonomy & Explanation without actionability taxonomy \\ \hline
\multirow{Health} & Articulation & \begin{tabular}[c]{@{}l@{}}-Most users found the explanations clear, concise, and useful.\\ -Some users suggested that practical advice and examples should\\  be included to help users understand medical terms.\\ -A few users mentioned that the language could be more\\  understandable to the colloquial mind.\end{tabular} & \begin{tabular}[c]{@{}l@{}}-Users generally found the explanations easy to understand in terms\\  of numbers but would benefit from examples and more practical advice.\\ -Some users pointed out that certain aspects were not well articulated,\\  such as age and gender information.\\ -A few users mentioned that the explanations did not justify the reasons \\ behind the recommendations, and some of the recommendations did \\ not make sense.\end{tabular} \\
 & Acceptability & \begin{tabular}[c]{@{}l@{}}-Users generally found the explanations acceptable.\\ -Some users pointed out the lack of examples and practical advice.\\ -A few users found the information too generic and not personalized\\  enough for the patient.\\ -One user mentioned that the closing comments in Case 2 were\\  insensitive.\end{tabular} & \begin{tabular}[c]{@{}l@{}}-Users generally found the explanations to be too complex or filled\\  with technical details that might not be easily understood by the patients.\\ -Some users highlighted that the explanations included impossible \\ or inappropriate recommendations, such as changing one's age or sex.\\ -A few users found the explanations acceptable but suggested more\\  explanation and detail.\end{tabular} \\
 & Feasibility & \begin{tabular}[c]{@{}l@{}}-Most users found the explanations feasible but suggested the need\\  for more practical advice and examples.\\ -Some users mentioned that the explanations would be more \\ feasible with further explanation from a doctor.\\ -One user pointed out the lack of consideration for the patient's\\  lifestyle or medical history.\end{tabular} & \begin{tabular}[c]{@{}l@{}}-Most users found the explanations to be unfeasible due to the \\ inclusion of impossible or inappropriate recommendations.\\ -Some users mentioned that the explanations did not provide \\ any guidance on how to achieve the targets set.\\ -One user commented on the lack of information on how \\ the data was generated.\end{tabular} \\
 & Sensitivity & \begin{tabular}[c]{@{}l@{}}-Many users felt that the explanations lacked personalization\\  and ethical considerations.\\ -Some users mentioned the need for considering personal \\ circumstances, genetic conditions, medical history, and lifestyle habits.\\ -A few users found the explanations non-biased.\end{tabular} & \begin{tabular}[c]{@{}l@{}}-Many users felt that the explanations lacked personalization and \\ did not take into consideration the personal characteristics of the patients.\\ -Some users pointed out that suggesting the change of sex or \\ lowering age is inappropriate and insensitive.\\ -A few users found the explanations to be impersonal and lacking\\  in addressing sensitive personal characteristics.\end{tabular} \\ \hline
\multirow{Finance} & Articulation & \begin{tabular}[c]{@{}l@{}}-Users found that the lack of feature weighting in the explainer\\  algorithm led to unnatural and confusing explanations.\\  For instance, users were unclear about the\\  relationship between renting and risk levels, as well as\\  the employment length expressed as an ambiguous number.\\ -Incorporating feature importance and providing clearer, more\\  intuitive explanations should be considered to improve articulation.\end{tabular} & \begin{tabular}[c]{@{}l@{}}-Varying levels of clarity in the explanations\\ -Some statements are nonsensical or impossible to follow\\ -Lack of underlying reasoning provided\\ -Formatting and articulation issues affecting comprehension\end{tabular} \\
 & Acceptability & \begin{tabular}[c]{@{}l@{}}-Users criticized the rationality behind certain recommendations,\\  such as reducing\\  income or the number of years employed. The need for feature\\  weighting and rationality\\  in the explainer algorithm is crucial for providing acceptable\\  and meaningful explanations.\end{tabular} & \begin{tabular}[c]{@{}l@{}}-Some recommendations are counterintuitive or hard to believe\\ -Certain advice is considered ridiculous or detrimental\\ -Users may not understand the reasoning behind the advice provided\\ -In some instances, users disagree with AI's recommendations\end{tabular} \\
 & Feasibility & \begin{tabular}[c]{@{}l@{}}-Users highlighted that some recommendations, such as \\  changing home ownership to rent or reducing income, \\ were not feasible or had negative consequences.\\ -Ensuring that counterfactual explanations are grounded\\  in real-world conditions is essential for providing valuable\\  and actionable advice.\end{tabular} & \begin{tabular}[c]{@{}l@{}}-Some recommendations are impossible or challenging to follow\\ -Users question the feasibility of certain advice given\\ -Users desire more personalization and rational suggestions\\ -Users point out that some of the advice may require lying or \\ changing circumstances\end{tabular} \\
 & Sensitivity & \begin{tabular}[c]{@{}l@{}}-Users found the lack of personalization and consideration\\  of personal characteristics uncomfortable and untrustworthy.\\ -Addressing factors such as age, employment, and income \\ in a sensitive and personalized manner is vital for ethical and \\ effective counterfactual explanations.\end{tabular} & \begin{tabular}[c]{@{}l@{}}-Users feel that some explanations lack sensitivity or understanding\\  of personal implications\\ -Potential negative side effects are not disclosed to the user\\ -Users express concerns over being told to be untruthful or \\ perform impossible tasks\\ -Users feel there is a lack of consideration for personal characteristics\\  and ethical concerns\end{tabular} \\ \hline
\multirow{Education} & Articulation & \begin{tabular}[c]{@{}l@{}}- Clear explanations for some users, while others find \\   explanations lacking\\ -Users request more strategies, examples, and further explanations\\ -Some explanations seem simplistic or convoluted\\ -Punctuation errors or lack of detail affect understanding\\  Users feel some explanations are demoralizing\end{tabular} & \begin{tabular}[c]{@{}l@{}}-Some users find explanations clear, coherent, and jargon-free\\ -Others consider explanations blunt, emotionless, or not related\\  to the real world\\ -Users are skeptical about the specificity of some advice\\ -Some find the advice too wordy or minimal\end{tabular} \\
 & Acceptability & \begin{tabular}[c]{@{}l@{}}-Explanations provide goals but lack actionable advice or strategies\\ -Users question the accuracy or relevance of some reasons given\\ -Some users find the information acceptable, while others feel \\  it is unsatisfying\\ -Users express concerns about consistency and evidence behind\\  the advice some users appreciate the fact-based nature of the\\  statements\end{tabular} & \begin{tabular}[c]{@{}l@{}}-Users find some explanations drastic or impossible to implement,\\  such as changing gender or parents' education level\\ -Many consider the advice unhelpful or harsh\\ -Some users express confusion or uncertainty about the AI's \\  suggestions\\ -Users describe some explanations as illogical, inappropriate, or rude\end{tabular} \\
 & Feasibility & \begin{tabular}[c]{@{}l@{}}-Users find some goals understandable and feasible, but lack \\  specific strategies\\ -Users question the impact of factors like age or gender on scores\\ -Trust in AI's results varies among users\end{tabular} & \begin{tabular}[c]{@{}l@{}}-Users question the feasibility of changing factors such as\\  parental education or gender\\ -Some users believe the AI's advice could be beneficial to\\  a certain extent\\ -Users express concerns about the difficulty of reaching \\ certain targets without guidance\\ -Some users find the advice irrelevant or not based on \\ individual potential\end{tabular} \\
 & Sensitivity & \begin{tabular}[c]{@{}l@{}}-Users feel some explanations lack sensitivity or understanding of \\ personal implications\\ -Users express concerns about the focus on factors that cannot be\\  changed, such as age, gender, or parental education\\ -Some users appreciate the factual nature of the statements\\ -Users question the focus on external factors rather than personal\\  attributes-Users find some explanations ethical or factual, while\\  others interpret them as potentially offensive\end{tabular} & \begin{tabular}[c]{@{}l@{}}-Users find some explanations insensitive, unethical, or impersonal\\ -Many express concerns about the AI's focus on factors outside\\  the individual's control, such as parents or gender\\ -Users describe some advice as unfair or lacking consideration\\  for personal circumstances\\ -Some users are indifferent to the explanations' sensitivity\end{tabular} \\ \hline
\end{tabular}
\caption{Comparison between feedback on generated explanations by employing actionability taxonomy and without it }
\label{tab:cfgencomp}
\end{table*}
\begin{table*}[]
\centering
\begin{tabular}{ll}
\hline
Domain & General Takeaways \\ \hline
Health & \begin{tabular}[c]{@{}l@{}}-Further explanations/ examples and strategies on HOW\\ -Ethical / Sensitivity\\ -More personalisation\\ -Considering patient history\\ -Causal and factual explanations also needed to make it\\  clear WHY happend and WHY counter would work\end{tabular} \\ \hline
Finance & \begin{tabular}[c]{@{}l@{}}-Further explanations/ examples and strategies on HOW\\ -Weighting features and considering rationality\\ -lack of considering feature feasibility level led to being\\ UNTRUSTWORTHY and UNNATURAL\\ -Sensitivity could be completely different from person to person\\ -Mentioning potential side effects\end{tabular} \\ \hline
Education & \begin{tabular}[c]{@{}l@{}}-Further explanations/ examples and strategies on HOW\\ -Factual explanation on:\\  * Why happend\\  * Why this suggestion is pertinent and related\\  * explain the impact and why mentioning not-actionables\\ - Sensitivity; lack of sensitivity makes explanations sound blunt and emotion less\end{tabular} \\ \hline
\end{tabular}
\caption{General key points from users for each domain}
\label{tab:genKeys}
\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\begin{tabular}{lll}
\hline
Domain & Metric & Performance \\ \hline
\multirow{Health} & Articulation & Not significant \\
 & Acceptability & Not significant \\
 & Feasibility & Not significant \\
 & Sensitivity & Significant \\ \hline
\multirow{Finance} & Articulation & Significant \\
 & Acceptability & Not significant \\
 & Feasibility & Not significant \\
 & Sensitivity & Significant \\ \hline
\multirow{Education} & Articulation & Significant \\
 & Acceptability & Not significant \\
 & Feasibility & Not significant \\
 & Sensitivity & Not significant \\ \hline
\end{tabular}
\caption{Performance}
\label{tab:signif}
\end{table*}

% \begin{itemize}
%     \item \textbf{feasibility Knowledge:} This theme appeared across health, finance, and education domains, with users preferring actionable guidance, including examples or strategies. Explanations offering concrete steps or advice for improvement lead to users feeling empowered and better prepared for informed decision-making.
%     \item \textbf{Handling Protected Features:} Across health, finance, and education domains, users were concerned about sensitive or personal features in explanations. This highlights the need to consider individual preferences, ethical concerns, and cultural sensitivities for age, sex, or other protected attributes. Personalised explanations addressing these issues can enhance the user experience by being more respectful and satisfying.
%     \item \textbf{Hybrid Explanation:} This theme emerged in the health and education domains, where users valued explanations that combined causal, factual, and counterfactual elements. By integrating different types of explanations, AI systems can provide users with a more comprehensive understanding of the underlying factors and relationships at play. Offering a diverse range of information can enhance clarity and contribute to a more satisfying user experience.
%     \item \textbf{Personalised Revision of Counterfactuals:} In the finance domain, users emphasized the need to consider individual constraints in counterfactual explanations. This necessitates generating alternative counterfactuals that account for users' unique circumstances and limitations, allowing AI systems to provide tailored, feasible recommendations better suited to each individual's needs.
%     \item \textbf{feasibility Impact:} Finance domain users desired explanations addressing potential impacts and side effects of suggested changes. By including information on the consequences of recommendations, AI systems can assist users in evaluating options and making informed decisions, highlighting the importance of understanding the broader implications of their actions.
%     \item \textbf{Structure and Context:} Users across the health, finance, and education domains emphasized the importance of clear and coherent writing, brevity, and the use of jargon-free language. Additionally, users valued explanations that were concise yet informative, providing an appropriate level of detail without being overly wordy or complex.
% \end{itemize}
